SCOT: Self-Supervised Contrastive Pretraining For Zero-Shot Compositional Retrieval

Compositional image retrieval (CIR) is a multimodal learning task where a model combines a query image with a user-provided text modification to retrieve a target image. CIR finds applications in a variety of domains including product retrieval (e-commerce) and web search. Existing methods primarily focus on fully-supervised learning, wherein models are trained on datasets of labeled triplets such as FashionIQ and CIRR. This poses two significant challenges: (i) curating such triplet datasets is labor intensive; and (ii) models lack generalization to unseen objects and domains. In this work, we propose SCOT (Self-supervised COmpositional Training), a novel zero-shot compositional pretraining strategy that combines existing large image-text pair datasets with the generative capabilities of large language models to contrastively train an embedding composition network. Specifically, we show that the text embedding from a large-scale contrastively-pretrained vision-language model can be utilized as proxy target supervision during compositional pretraining, replacing the target image embedding. In zero-shot settings, this strategy surpasses SOTA zero-shot compositional retrieval methods as well as many fully-supervised methods on standard benchmarks such as FashionIQ and CIRR.

==> tables/CIRR_main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
%\setlength{\tabcolsep}{4.5pt}
\centering
\fontsize{7.2pt}{7.2pt}\selectfont
\begin{tabular}{llcccccccc}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & \multicolumn{4}{c}{\textbf{Recall@K}} & \multicolumn{3}{c}{\textbf{Recall$_{\text{subset}}$@K}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
 & & & \( K = 1 \) & \( K = 5 \) & \( K = 10 \) & \( K = 50 \) & \( K = 1 \) & \( K = 2 \) & \( K = 3 \) \\
\midrule
\multirow{4}{*}{Supervised}
& MAAF \cite{maaf} & Multi & 10.31 & 33.03 & 48.30 & 80.06 & 21.05 & 41.81 & 61.60 \\ % MAAF (as reported in CIRPLANT paper) is the original version, which uses ResNet image features, and LSTM text features
& CIRPLANT \cite{CIRR} & OSCAR & 19.55 & 52.55 & 68.39 & 92.38 & 39.20 & 63.03 & 79.49 \\ % CIRPLANT uses OSCAR, which takes as input ResNet image features and directly tokenizes and embeds the text. We could also just put "Multi" as the backbone, given that the ResNet is involved, but I think OSCAR is more informative and clear enough.
& CLIP4CIR \cite{combinerarch} & CLIP-L & 33.59 & 65.35 & 77.35 & 95.21 & 62.39 & 81.81 & 92.02 \\
& BLIP4CIR \cite{BLIP4Cir} & BLIP & 40.15 & 73.08 & 83.88 & 96.27 & 72.10 & 88.27 & 95.93 \\
\midrule
\multirow{7}{*}{Zero-Shot} 

& Image-only & CLIP-B & 6.94 & 22.94 & 33.71 & 59.18 & 21.06 & 41.01 & 60.34\\
& Text-only & CLIP-B & 21.16 & 45.35 & 57.40 & 81.06 & 62.26 & 81.08 & 90.75 \\
& Image+Text & CLIP-B & 10.46 & 32.41 & 46.39 & 75.11 & 30.09 & 54.24 & 73.20\\

& Image-only & CLIP-L & 7.47 & 23.88 & 34.07 & 57.57 & 20.87 & 41.95 & 61.13\\
& Text-only & CLIP-L & 22.00 & 45.79 & 57.57 & 79.59 & 61.71 & 80.26 & 90.43 \\
& Image+Text & CLIP-L & 10.55 & 32.70 & 45.71 & 74.26 & 31.06 & 55.69 & 73.93\\

& Image-only & BLIP-2 & 7.59 & 24.43 & 35.56 & 61.42 & 20.74 & 40.67 & 61.08 \\
& Text-only & BLIP-2 & 33.52	& 61.50 & 71.35 & 88.31 & 72.53 & 88.02 & 94.87 \\
& Image+Text & BLIP-2 & 19.69 & 49.98 & 64.39 & 90.01 & 45.69 & 71.18 & 85.83 \\

& PALAVRA \cite{PALAVRA} & CLIP-B & 16.62 & 43.49 & 58.51 & 83.95 & 41.61 & 65.30 & 80.94 \\
& TransAgg* \cite{transagg} & CLIP-B & 24.46 & 53.61 & 67.54 & 89.81 & 57.81 & 78.17 & 89.54 \\
& TransAgg* \cite{transagg} & CLIP-L & 25.04 & 53.98 & 67.59 & 88.94 & 55.33 & 76.82 & 88.94\\
& TransAgg* \cite{transagg} & BLIP & 34.89 & 64.75 & 76.24 & 92.22 & 66.34 & 83.76 & 92.92\\
& SEARLE\textsuperscript{\textdagger} \cite{SEARLE} & CLIP-B & 24.00 & 53.42 & 66.82 & 89.78 & 54.89 & 76.60 & 88.19\\
& SEARLE-XL\textsuperscript{\textdagger} \cite{SEARLE} & CLIP-L & 24.24 & 52.48 & 66.29 & 88.84 & 53.76 & 75.01 & 88.19 \\
% & SEARLE-XL-OTI \cite{SEARLE} & & 24.87 & 52.31 & 66.29 & 88.58 & 53.80 & 74.31 & 86.94 \\
& Pic2Word \cite{Saito_2023_CVPR} & CLIP-L & 23.9 & 51.7 & 65.3 & 87.8 & - & - & - \\
& \textbf{SCOT (Ours)} & CLIP-B & 22.80 & 53.18 & 66.22 & 89.64 & 53.25 & 75.45 & 88.31 \\
& \textbf{SCOT (Ours)} & CLIP-L & 24.36 & 53.52 & 67.37 & 89.35 & 51.47 & 74.24 & 87.90 \\
& \textbf{SCOT (Ours)} & BLIP-2 & \textbf{36.82} & \textbf{64.34} & \textbf{74.48} & \textbf{93.42} & \textbf{75.73} & \textbf{88.70} & \textbf{94.84} \\
\bottomrule
\end{tabular}
\vspace{0.2em}
\caption{
    \textbf{Results on CIRR.}
    %$\text{*}$ are the results reported by the authors.
    The bottom portion of the table presents zero-shot results from our proposed approach compared against existing zero-shot methods, while the top portion presents results from existing fully-supervised approaches. *TransAgg results using frozen backbones. \textsuperscript{\textdagger}SEARLE results from inversion model. See supplementary material for more results.
}
\label{table:cirr}
\vspace{-1.0em}
\end{table*}

==> tables/CIRR_main_results_new_order_cirrcheckpointed.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
%\setlength{\tabcolsep}{4.5pt}
\centering
\fontsize{7.2pt}{7.2pt}\selectfont
\begin{tabular}{lllccccccc}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & \multicolumn{4}{c}{\textbf{Recall@K}} & \multicolumn{3}{c}{\textbf{Recall$_{\text{subset}}$@K}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-10}
 & & & \( K = 1 \) & \( K = 5 \) & \( K = 10 \) & \( K = 50 \) & \( K = 1 \) & \( K = 2 \) & \( K = 3 \) \\
\midrule
\multirow{4}{*}{Supervised}
& MAAF \cite{maaf} & Multi & 10.31 & 33.03 & 48.30 & 80.06 & 21.05 & 41.81 & 61.60 \\ % MAAF (as reported in CIRPLANT paper) is the original version, which uses ResNet image features, and LSTM text features
& CIRPLANT \cite{CIRR} & OSCAR & 19.55 & 52.55 & 68.39 & 92.38 & 39.20 & 63.03 & 79.49 \\ % CIRPLANT uses OSCAR, which takes as input ResNet image features and directly tokenizes and embeds the text. We could also just put "Multi" as the backbone, given that the ResNet is involved, but I think OSCAR is more informative and clear enough.
& CLIP4CIR \cite{combinerarch} & CLIP-L & 33.59 & 65.35 & 77.35 & 95.21 & 62.39 & 81.81 & 92.02 \\
& BLIP4CIR \cite{BLIP4Cir} & BLIP & 40.15 & 73.08 & 83.88 & 96.27 & 72.10 & 88.27 & 95.93 \\
\midrule
\multirow{18}{*}{Zero-Shot} 

& Image-only & CLIP-L & 7.47 & 23.88 & 34.07 & 57.57 & 20.87 & 41.95 & 61.13\\
& Text-only & CLIP-L & 22.00 & 45.79 & 57.57 & 79.59 & \textbf{61.71} & \textbf{80.26} & \textbf{90.43} \\
& Image+Text & CLIP-L & 10.55 & 32.70 & 45.71 & 74.26 & 31.06 & 55.69 & 73.93\\
& Pic2Word \cite{Saito_2023_CVPR} & CLIP-L & 23.9 & 51.7 & 65.3 & 87.8 & - & - & - \\
% & SEARLE-XL-OTI \cite{SEARLE} & & 24.87 & 52.31 & 66.29 & 88.58 & 53.80 & 74.31 & 86.94 \\
& SEARLE-XL \cite{SEARLE} & CLIP-L & 24.24 & 52.48 & 66.29 & 88.84 & 53.76 & 75.01 & 88.19 \\
& TransAgg\cite{transagg} & CLIP-L & 25.04 & 53.98 & 67.59 & 88.94 & 55.33 & 76.82 & 88.94\\
& SCOT (Ours) & CLIP-L & 24.36 & 53.52 & 67.37 & \textbf{89.35} & 51.47 & 74.24 & 87.90 \\

\cmidrule(lr){2-10}

& Image-only & CLIP-B & 6.94 & 22.94 & 33.71 & 59.18 & 21.06 & 41.01 & 60.34\\
& Text-only & CLIP-B & 21.16 & 45.35 & 57.40 & 81.06 & \textbf{62.26} & \textbf{81.08} & \textbf{90.75} \\
& Image+Text & CLIP-B & 10.46 & 32.41 & 46.39 & 75.11 & 30.09 & 54.24 & 73.20\\
& PALAVRA \cite{PALAVRA} & CLIP-B & 16.62 & 43.49 & 58.51 & 83.95 & 41.61 & 65.30 & 80.94 \\
& SEARLE \cite{SEARLE} & CLIP-B & 24.00 & 53.42 & 66.82 & 89.78 & 54.89 & 76.60 & 88.19\\
& TransAgg\textsuperscript{\textdagger} \cite{transagg} & CLIP-B & \textbf{24.46} & \textbf{53.61} & \textbf{67.54} & \textbf{89.81} & 57.81 & 78.17 & 89.54 \\
& SCOT (Ours) & CLIP-B & 22.80 & 53.18 & 66.22 & 89.64 & 53.25 & 75.45 & 88.31 \\

\cmidrule(lr){2-10}

& Image-only & BLIP & 34.19 & 61.68 & 71.74 & 87.83 & \textbf{72.34} & \textbf{87.97} & \textbf{94.79} \\
& Text-only & BLIP & 7.23 & 25.78 & 37.35 & 62.34 & 20.60 & 40.96 & 61.35 \\
& Image+Text & BLIP & 8.24 & 28.96 & 41.23 & 68.07 & 23.64 & 45.35 & 66.29 \\
& TransAgg \cite{transagg} & BLIP & \underline{34.89} & \underline{64.75} & \underline{76.24} & \underline{92.22} & \underline{66.34} & \underline{83.76} & \underline{92.92} \\
& SCOT (Ours) & BLIP & \textbf{36.31} & \textbf{66.19} & \textbf{77.37} & \textbf{92.96} & 64.73 & 83.20 & 92.15 \\

\cmidrule(lr){2-10}

& Image-only & BLIP-2 & 7.59 & 24.43 & 35.56 & 61.42 & 20.74 & 40.67 & 61.08 \\
& Text-only & BLIP-2 & \underline{33.52} & \underline{61.50} & \underline{71.35} & \underline{88.31} & \underline{72.53} & \underline{88.02} & \textbf{94.87} \\
& Image+Text & BLIP-2 & 19.69 & 49.98 & 64.39 & 90.01 & 45.69 & 71.18 & 85.83 \\
& SCOT (Ours) & BLIP-2 & \textbf{36.82} & \textbf{64.34} & \textbf{74.48} & \textbf{93.42} & \textbf{75.73} & \textbf{88.70} & 94.84 \\
\bottomrule
\end{tabular}
\vspace{0.2em}
\caption{
    \textbf{Results on CIRR.}
    %$\text{*}$ are the results reported by the authors.
    The bottom portion of the table presents zero-shot results from our proposed approach compared against existing zero-shot methods, while the top portion presents results from existing fully-supervised approaches. *SEARLE results from inversion model. \textsuperscript{\textdagger}TransAgg results using frozen backbones. See supplementary material for more results.
}
\label{table:cirr}
\vspace{-1.0em}
\end{table*}

==> tables/backbone_table.tex <==
% \begin{table*}[ht!]
% \centering
% \begin{tabular}{clccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Top/Tee}} & \multirow{2}{*}{\textbf{FIQ}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
% & & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & \\
% \midrule
% \multirow{4}{*}{CLIP B/32}
% & Image-Only & 5.88 & 13.19 &  6.96 & 14.08 & 4.46 & 11.89 & 6.22 & 13.61 & \\ 
% & Text-Only & 18.41 & 36.28 & 14.92 & 33.81 & 19.77 & 34.69 & 20.55 & 40.33 & \\
% & Image+Text & 13.36 & 27.51 &  12.44 & 28.55 & 12.61 & 24.82 & 15.04 & 29.16 & \\
% & SCOT & 24.14 & 43.44 & 19.73 & 41.24 & 25.51 & 42.93 & 27.18 & 46.14 &  \\
% \midrule
% \multirow{4}{*}{CLIP L/14}
% & Image-Only & 7.97 & 17.43 & 5.25 & 13.63 & 10.54 & 20.65 & 8.10 & 18.01 \\ 
% & Text-Only & 19.01 & 35.26 & 15.22 & 33.01 & 19.82 & 33.31 & 21.87 & 39.46\\
% & Image + Text & 18.12 & 33.17 & 14.27 & 31.33 & 19.13 & 32.28 & 20.95 & 35.90\\
% & \textbf{SCOT} & \textbf{28.27} & \textbf{47.44} & \textbf{23.69} & \textbf{45.06} & \textbf{29.09} & \textbf{47.01} & \textbf{32.02} & \textbf{50.33} & \textbf{37.86} \\
% \midrule
% % \multirow{4}{*}{CLIP R50x4}
% % & Image-Only & - & - &  - & - &  - &  - &  - & - & \\ 
% % & Text-Only & - & - &  - & - &  - &  - &  - & - & \\
% % & Image+Text & - & - &  - & - &  - &  - &  - & - & \\
% % & SCOT & - & - &  - & - &  - &  - &  - & - &  \\
% % \midrule
% \multirow{4}{*}{BLIP-2}
% & Image-Only & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 & 12.73 \\
% & Text Only & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31 & 34.13 \\
% & Image + Text & 29.21 & 50.05 & 23.3 & 45.61 & 32.82 & \underline{53.09} & 31.51 & 51.45 & 39.63 \\
% & \textbf{SCOT (Ours)} & \textbf{38.45} & \textbf{60.03} & \textbf{32.78} & \textbf{55.91} & \textbf{41.42} & \textbf{61.09} & \textbf{41.15} & \textbf{63.1} & \textbf{49.24} \\
% \bottomrule
% \end{tabular}
% \caption{Zero-shot Results on FashionIQ with varying backbones}
% \label{table:different_backbones}
% \end{table*}

% \begin{table*}[ht!]
% \centering
% \begin{tabular}{clccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Top/Tee}} & \multirow{2}{*}{\textbf{FIQ}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
% & & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & \\
% \midrule
% \multirow{4}{*}{CLIP B/32}
% & Image-Only & 5.88 & 13.19 &  6.96 & 14.08 & 4.46 & 11.89 & 6.22 & 13.61 & \\ 
% & Text-Only & 18.41 & 36.28 & 14.92 & 33.81 & 19.77 & 34.69 & 20.55 & 40.33 & \\
% & Image+Text & 13.36 & 27.51 &  12.44 & 28.55 & 12.61 & 24.82 & 15.04 & 29.16 & \\
% & SCOT & 24.14 & 43.44 & 19.73 & 41.24 & 25.51 & 42.93 & 27.18 & 46.14 &  \\
% \midrule
% \multirow{4}{*}{CLIP L/14}
% & Image-Only & 7.97 & 17.43 & 5.25 & 13.63 & 10.54 & 20.65 & 8.10 & 18.01 \\ 
% & Text-Only & 19.01 & 35.26 & 15.22 & 33.01 & 19.82 & 33.31 & 21.87 & 39.46\\
% & Image + Text & 18.12 & 33.17 & 14.27 & 31.33 & 19.13 & 32.28 & 20.95 & 35.90\\
% & \textbf{SCOT} & \textbf{28.27} & \textbf{47.44} & \textbf{23.69} & \textbf{45.06} & \textbf{29.09} & \textbf{47.01} & \textbf{32.02} & \textbf{50.33} & \textbf{37.86} \\
% \midrule
% % \multirow{4}{*}{CLIP R50x4}
% % & Image-Only & - & - &  - & - &  - &  - &  - & - & \\ 
% % & Text-Only & - & - &  - & - &  - &  - &  - & - & \\
% % & Image+Text & - & - &  - & - &  - &  - &  - & - & \\
% % & SCOT & - & - &  - & - &  - &  - &  - & - &  \\
% % \midrule
% \multirow{4}{*}{BLIP-2}
% & Image-Only & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 & 12.73 \\
% & Text Only & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31 & 34.13 \\
% & Image + Text & 29.21 & 50.05 & 23.3 & 45.61 & 32.82 & \underline{53.09} & 31.51 & 51.45 & 39.63 \\
% & \textbf{SCOT (Ours)} & \textbf{38.45} & \textbf{60.03} & \textbf{32.78} & \textbf{55.91} & \textbf{41.42} & \textbf{61.09} & \textbf{41.15} & \textbf{63.1} & \textbf{49.24} \\
% \bottomrule
% \end{tabular}
% \caption{Zero-shot Results on FashionIQ with varying backbones}
% \label{table:different_backbones}
% \end{table*}

\begin{table}[t]
\centering
\fontsize{7.7pt}{7.7pt}\selectfont
\begin{tabular}{lp{2.5cm}r{1cm}r{1cm}r{1cm}r{1cm}r{1cm}r{1cm}r{1cm}}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{FashionIQ}} & \multicolumn{4}{c}{\textbf{CIRR}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-9} & & \( R @ 10 \) & \( R @ 50 \) & \( FIQ \) & \( R @ 1 \) & \( R @ 5 \) & \( R @ 10 \) & \( R @ 50 \) \\
\midrule
\multirow{4}{*}{CLIP B/32}
& Image-Only  & -12.53 & -23.09 & -17.81 & -14.22 & -22.41 & -23.69 & -21.88 \\
& Image+Text  & -5.05  & -8.77  & -6.91  & -10.70 & -12.94 & -11.01 & -5.95  \\
& PALAVRA     & +1.35  & +0.97  & +1.16  & -4.54  & -1.86  & +1.11  & +2.89  \\
& SEARLE*     & +4.48  & +6.25  & +5.37  & +2.84  & +8.07  & +9.42  & +8.72  \\
& TransAgg    & +5.50  & +8.40  & +6.95  & +3.30  & +8.26  & +10.14 & +8.75  \\
& SCOT (Ours) & +5.73  & +7.16  & +6.45  & +1.64  & +7.83  & +8.82  & +8.58  \\

\midrule

\multirow{4}{*}{CLIP L/14}
& Image-Only  & -11.04 & -17.83 & -14.44 & -14.53 & -21.91 & -23.50 & -22.02 \\
& Image+Text  & -0.89  & -2.09  & -1.49  & -11.45 & -13.09 & -11.86 & -5.33  \\
& Pic2Word    & +5.69  & +8.44  & +7.07  & +1.90  & +5.91  & +7.73  & +8.21  \\
& SEARLE-XL   & +6.55  & +10.97 & +8.76  & +2.24  & +6.69  & +8.72  & +9.25  \\
& TransAgg    & +9.56  & +13.03 & +11.30 & +3.04  & +8.19  & +10.02 & +9.35  \\
& SCOT (Ours) & +9.26  & +12.18 & +10.72 & +2.36  & +7.73  & +9.80  & +9.76  \\

\midrule
\multirow{4}{*}{BLIP}
& Image-Only  & -17.36 & -27.33 & -22.35 & -26.96 & -35.90 & -34.39 & -25.49 \\
& Image+Text  & -15.95 & -24.57 & -20.26 & -25.95 & -32.72 & -30.51 & -19.76 \\
& TransAgg    & +2.94  & +3.37  & +3.16  & +0.70  & +3.07  & +4.50  & +4.39  \\
& SCOT (Ours) & +6.67  & +8.60  & +7.64  & +2.12  & +4.51  & +5.63  & +5.13  \\
\midrule
\multirow{4}{*}{BLIP-2}
& Image-Only  & -17.15 & -25.66 & -21.41 & -25.93 & -37.07 & -35.79 & -26.89 \\
& Image+Text  & +4.53  & +6.46  & +5.50  & -13.83 & -11.52 & -6.96  & +1.70  \\
& SCOT (Ours) & +13.77 & +16.44 & +15.11 & +3.30  & +2.84  & +3.13  & +5.11 \\
\bottomrule
\end{tabular}
\vspace{1em}
\caption{\textbf{Ablation on relative improvement over Text-Only performance across backbones:} Zero-shot results of our approach on FashionIQ and CIRR}
\label{table:different_backbones}
\vspace{-1.0em}
\end{table}


==> tables/backbone_table_old.tex <==
% \begin{table*}[ht!]
% \centering
% \begin{tabular}{clccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Top/Tee}} & \multirow{2}{*}{\textbf{FIQ}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
% & & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & \\
% \midrule
% \multirow{4}{*}{CLIP B/32}
% & Image-Only & 5.88 & 13.19 &  6.96 & 14.08 & 4.46 & 11.89 & 6.22 & 13.61 & \\ 
% & Text-Only & 18.41 & 36.28 & 14.92 & 33.81 & 19.77 & 34.69 & 20.55 & 40.33 & \\
% & Image+Text & 13.36 & 27.51 &  12.44 & 28.55 & 12.61 & 24.82 & 15.04 & 29.16 & \\
% & SCOT & 24.14 & 43.44 & 19.73 & 41.24 & 25.51 & 42.93 & 27.18 & 46.14 &  \\
% \midrule
% \multirow{4}{*}{CLIP L/14}
% & Image-Only & 7.97 & 17.43 & 5.25 & 13.63 & 10.54 & 20.65 & 8.10 & 18.01 \\ 
% & Text-Only & 19.01 & 35.26 & 15.22 & 33.01 & 19.82 & 33.31 & 21.87 & 39.46\\
% & Image + Text & 18.12 & 33.17 & 14.27 & 31.33 & 19.13 & 32.28 & 20.95 & 35.90\\
% & \textbf{SCOT} & \textbf{28.27} & \textbf{47.44} & \textbf{23.69} & \textbf{45.06} & \textbf{29.09} & \textbf{47.01} & \textbf{32.02} & \textbf{50.33} & \textbf{37.86} \\
% \midrule
% % \multirow{4}{*}{CLIP R50x4}
% % & Image-Only & - & - &  - & - &  - &  - &  - & - & \\ 
% % & Text-Only & - & - &  - & - &  - &  - &  - & - & \\
% % & Image+Text & - & - &  - & - &  - &  - &  - & - & \\
% % & SCOT & - & - &  - & - &  - &  - &  - & - &  \\
% % \midrule
% \multirow{4}{*}{BLIP-2}
% & Image-Only & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 & 12.73 \\
% & Text Only & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31 & 34.13 \\
% & Image + Text & 29.21 & 50.05 & 23.3 & 45.61 & 32.82 & \underline{53.09} & 31.51 & 51.45 & 39.63 \\
% & \textbf{SCOT (Ours)} & \textbf{38.45} & \textbf{60.03} & \textbf{32.78} & \textbf{55.91} & \textbf{41.42} & \textbf{61.09} & \textbf{41.15} & \textbf{63.1} & \textbf{49.24} \\
% \bottomrule
% \end{tabular}
% \caption{Zero-shot Results on FashionIQ with varying backbones}
% \label{table:different_backbones}
% \end{table*}

% \begin{table*}[ht!]
% \centering
% \begin{tabular}{clccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Top/Tee}} & \multirow{2}{*}{\textbf{FIQ}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
% & & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & \\
% \midrule
% \multirow{4}{*}{CLIP B/32}
% & Image-Only & 5.88 & 13.19 &  6.96 & 14.08 & 4.46 & 11.89 & 6.22 & 13.61 & \\ 
% & Text-Only & 18.41 & 36.28 & 14.92 & 33.81 & 19.77 & 34.69 & 20.55 & 40.33 & \\
% & Image+Text & 13.36 & 27.51 &  12.44 & 28.55 & 12.61 & 24.82 & 15.04 & 29.16 & \\
% & SCOT & 24.14 & 43.44 & 19.73 & 41.24 & 25.51 & 42.93 & 27.18 & 46.14 &  \\
% \midrule
% \multirow{4}{*}{CLIP L/14}
% & Image-Only & 7.97 & 17.43 & 5.25 & 13.63 & 10.54 & 20.65 & 8.10 & 18.01 \\ 
% & Text-Only & 19.01 & 35.26 & 15.22 & 33.01 & 19.82 & 33.31 & 21.87 & 39.46\\
% & Image + Text & 18.12 & 33.17 & 14.27 & 31.33 & 19.13 & 32.28 & 20.95 & 35.90\\
% & \textbf{SCOT} & \textbf{28.27} & \textbf{47.44} & \textbf{23.69} & \textbf{45.06} & \textbf{29.09} & \textbf{47.01} & \textbf{32.02} & \textbf{50.33} & \textbf{37.86} \\
% \midrule
% % \multirow{4}{*}{CLIP R50x4}
% % & Image-Only & - & - &  - & - &  - &  - &  - & - & \\ 
% % & Text-Only & - & - &  - & - &  - &  - &  - & - & \\
% % & Image+Text & - & - &  - & - &  - &  - &  - & - & \\
% % & SCOT & - & - &  - & - &  - &  - &  - & - &  \\
% % \midrule
% \multirow{4}{*}{BLIP-2}
% & Image-Only & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 & 12.73 \\
% & Text Only & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31 & 34.13 \\
% & Image + Text & 29.21 & 50.05 & 23.3 & 45.61 & 32.82 & \underline{53.09} & 31.51 & 51.45 & 39.63 \\
% & \textbf{SCOT (Ours)} & \textbf{38.45} & \textbf{60.03} & \textbf{32.78} & \textbf{55.91} & \textbf{41.42} & \textbf{61.09} & \textbf{41.15} & \textbf{63.1} & \textbf{49.24} \\
% \bottomrule
% \end{tabular}
% \caption{Zero-shot Results on FashionIQ with varying backbones}
% \label{table:different_backbones}
% \end{table*}

\begin{table}[t]
\centering
\fontsize{7.7pt}{7.7pt}\selectfont
\begin{tabular}{lp{2.5cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{FashionIQ}} & \multicolumn{4}{c}{\textbf{CIRR}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-9} & & \( R @ 10 \) & \( R @ 50 \) & \( FIQ \) & \( R @ 1 \) & \( R @ 5 \) & \( R @ 10 \) & \( R @ 50 \) \\
\midrule
\multirow{4}{*}{CLIP B/32}
& Image-Only & 5.88 & 13.19 & 9.53 & 6.94 & 22.94 & 33.71 & 59.18 \\ 
& Text-Only & 18.41 & 36.28 & 27.34 & 21.16 & 45.35 & 57.40 & 81.06 \\
& Image + Text & 13.36 & 27.51 & 20.43 & 10.46 & 32.41 & 46.39 & 75.11 \\
& SCOT (Ours) & \textbf{24.14} & \textbf{43.44} & \textbf{33.79} & \textbf{22.80} & \textbf{53.18} & \textbf{66.22} & \textbf{89.64} \\
\midrule
\multirow{4}{*}{CLIP L/14}
& Image-Only & 7.97 & 17.43 & 12.7 & 7.47 & 23.88 & 34.07 & 57.57 \\ 
& Text-Only & 19.01 & 35.26 & 27.13 & 22.00 & 45.79 & 57.57 & 79.59 \\
& Image + Text & 18.12 & 33.17 & 25.64 & 10.55 & 32.70 & 45.71 & 74.26  \\
& SCOT (Ours) & \textbf{28.27} & \textbf{47.44} & \textbf{37.85} & \underline{24.36} & \underline{53.52} & \underline{67.37} & \textbf{89.35} \\
\midrule
\multirow{4}{*}{BLIP}
& Image-Only & 6.65 & 15.40 & 11.02 & 7.22 & 25.78 & 37.34 & 62.33  \\
& Text-Only & 24.01 & 42.73 & 66.74 & 34.19 &  61.68 & 71.73 & 87.83  \\
& Image + Text & 8.06 & 18.16 & 13.11 & 8.24 & 28.96 & 41.23 & 68.07  \\
& SCOT (Ours) & \textbf{30.68} & \textbf{51.33} & \textbf{41.01} & \textbf{36.31} & \textbf{66.19} & \textbf{77.37} & \textbf{92.96}  \\
\midrule
\multirow{4}{*}{BLIP-2}
& Image-Only & 7.53 & 17.93 & 12.73 & 7.59 & 24.43 & 35.56 & 61.42  \\
& Text-Only & 24.68 & 43.59 & 34.13 & 33.52 & 61.50 & 71.35 & 88.31  \\
& Image + Text & 29.21 & 50.05 & 39.63 & 19.69 & 49.98 & 64.39 & 90.01  \\
& SCOT (Ours) & \textbf{38.45} & \textbf{60.03} & \textbf{49.24} & \textbf{36.82} & \textbf{64.34} & \textbf{74.48} & \textbf{93.42}  \\
\bottomrule
\end{tabular}
\vspace{1em}
\caption{\textbf{Ablation on relative improvement over Text-Only performance across backbones:} Zero-shot results of our approach on FashionIQ and CIRR}
\label{table:different_backbones}
\vspace{-1.0em}
\end{table}


==> tables/fashionIQ_main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
% \setlength{\tabcolsep}{5.5pt}
\centering
\footnotesize
%\setlength{\tabcolsep}{2pt} % Default value: 6pt
\fontsize{7.2pt}{7.2pt}\selectfont
\begin{tabular}{@{}lccccccccccH@{}}

\toprule
\multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Top/Tee}} & \multirow{2}{*}{\textbf{FIQ}} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
& & & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & \\
\midrule
\multirow{4}{*}{Sup.}
& DCNet \cite{dcnet} & Multi & 30.44 & 58.29 & 28.95 & 56.07 & 23.95 & 47.30 & 30.44 & 58.29 & 44.37\\ 
& CLIP4CIR \cite{combinerarch} & CLIP-L & 38.32 & 61.74 & 33.81 & 59.40 & 39.99 & 60.45 & 41.41 & 65.37 & 50.03\\
& FashionVLP \cite{fashionVLP} & Multi & 34.27 & 62.51 & 32.42 & 60.29 & 31.89 & 58.44 & 38.51 & 68.79 & 48.39\\
& BLIP4CIR \cite{BLIP4Cir} & BLIP & 43.49 & 67.31 & 42.09 & 67.33 & 41.76 & 64.28 & 46.61 & 70.32 & 55.40\\
\midrule
\multirow{19}{*}{Z-S}
& Image-Only & CLIP-B & 5.88 & 13.19 &  6.96 & 14.08 & 4.46 & 11.89 & 6.22 & 13.61 \\ 
& Text-Only & CLIP-B & 18.41 & 36.28 & 14.92 & 33.81 & 19.77 & 34.69 & 20.55 & 40.33 \\
& Image+Text & CLIP-B & 13.36 & 27.51 &  12.44 & 28.55 & 12.61 & 24.82 & 15.04 & 29.16  \\
& Image-Only & CLIP-L  & 7.97 & 17.43 & 5.25 & 13.63 & 10.54 & 20.65 & 8.10 & 18.01  \\ 
& Text-Only & CLIP-L  & 19.01 & 35.26 & 15.22 & 33.01 & 19.82 & 33.31 & 21.87 & 39.46 \\
& Image+Text & CLIP-L & 18.12 & 33.17 & 14.27 & 31.33 & 19.13 & 32.28 & 20.95 & 35.90 \\
& Image-Only & BLIP-2 & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 \\
& Text Only & BLIP-2 & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31  \\
& Image+Text & BLIP-2 & 29.21 & 50.05 & 23.30 & 45.61 & 32.82 & 53.09 & 31.51 & 51.45  \\
\cmidrule(lr){2-11}
%& SEARLE-XL-OTI \cite{SEARLE} & CLIP-L & 27.61 & 47.90 & 21.57 & 44.47 & 30.37 & 47.49 & 30.90 & 51.76 & 37.75 \\
& PALAVRA \cite{PALAVRA} & CLIP-B & 19.76 & 37.25 & 17.25 & 35.94 & 21.49 & 37.05 & 20.55 & 38.76 & 28.50 \\
% & CompoDiff$\text{*}$ & \underline{37.36} & \underline{50.85} & \textbf{33.91} &\underline{47.85} & \underline{38.1} & 52.48 & \underline{40.07} & \underline{52.22} & \underline{44.10} \\
& Context-I2W \cite{tang2023context} & CLIP-L & 27.8 & 48.9 & 23.1 & 45.3 & 29.7 & 48.6 & 30.6 & 52.9 & 38.35 \\
& TransAgg* \cite{transagg} & CLIP-B & 23.91 & 44.68 & 19.44 & 42.04 & 25.37 & 42.69 & 26.93 & 49.31 & - \\
& TransAgg* \cite{transagg} & CLIP-L & 28.57 & 48.29 & 23.85 & 44.57 & 29.54 & 47.79 & 32.33 & 52.52 & - \\
& TransAgg* \cite{transagg} & BLIP & 26.95 & 46.10 & 21.67 & 41.89 & 28.07 & 45.63 & 31.11 & 50.79 & - \\
& SEARLE\textsuperscript{\textdagger} \cite{SEARLE} & CLIP-B & 22.89 & 42.53 & 18.54 & 39.51 & 24.44 & 41.61 & 18.54 & 39.51 \\
& SEARLE-XL\textsuperscript{\textdagger} \cite{SEARLE} & CLIP-L & 25.56 & 46.23 & 20.48 & 43.13 & 26.89 & 45.58 & 29.32 & 49.97 \\
& Pic2Word \cite{Saito_2023_CVPR} & CLIP-L & 24.7 & 43.7 & 20.0 & 40.2 & 26.2 & 43.6 & 27.9 & 47.4 & 34.2 \\
\cmidrule(lr){2-11}
& \textbf{SCOT (Ours)} & CLIP-B & \textbf{24.14} & \textbf{43.44} & \textbf{19.73} & \textbf{41.24} & \textbf{25.51} & \textbf{42.93} & \textbf{27.18} & \textbf{46.14} \\
& \textbf{SCOT (Ours)} & CLIP-L & \textbf{28.27} & \textbf{47.44} & \textbf{23.69} & \textbf{45.06} & \textbf{29.09} & \textbf{47.01} & \textbf{32.02} & \textbf{50.33}  \\
& \textbf{SCOT (Ours)} & BLIP-2 & \textbf{38.45} & \textbf{60.03} & \textbf{32.78} & \textbf{55.91} & \textbf{41.42} & \textbf{61.09} & \textbf{41.15} & \textbf{63.10} & \textbf{49.24} \\
\bottomrule
\end{tabular}
\vspace{0.2em}
\caption{\textbf{Results on FashionIQ.} 
The bottom portion of the table presents zero-shot results from our proposed approach compared against existing zero-shot methods, while the top portion presents results from existing fully-supervised approaches. *TransAgg results using frozen backbones. \textsuperscript{\textdagger}SEARLE results from inversion model. See supplementary material for more results.
}
\label{table:fashioniq}
\vspace{-1em}
\end{table*}

% & Image Only$^\dagger$ & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 & 12.73 \\
% & Text Only$^\dagger$ & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31 & 34.13 \\
% & Image + Text$^\dagger$ & 29.21 & 50.05 & 23.3 & 45.61 & 32.82 & \underline{53.09} & 31.51 & 51.45 & 39.63 \\

==> tables/fashionIQ_old_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
% \setlength{\tabcolsep}{5.5pt}
\centering
\footnotesize
%\setlength{\tabcolsep}{2pt} % Default value: 6pt
\fontsize{7.2pt}{7.2pt}\selectfont
\begin{tabular}{@{}lllccccccccH@{}}

\toprule
\multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Top/Tee}} & \multirow{2}{*}{\textbf{FIQ}} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
& & & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & $\boldsymbol{R @ 10}$ & $\boldsymbol{R @ 50}$ & \\
\midrule
\multirow{4}{*}{Sup.}
& DCNet \cite{dcnet} & Multi & 30.44 & 58.29 & 28.95 & 56.07 & 23.95 & 47.30 & 30.44 & 58.29 & 44.37\\ 
& FashionVLP \cite{fashionVLP} & Multi & 34.27 & 62.51 & 32.42 & 60.29 & 31.89 & 58.44 & 38.51 & 68.79 & 48.39\\
& CLIP4CIR \cite{combinerarch} & CLIP-L & 38.32 & 61.74 & 33.81 & 59.40 & 39.99 & 60.45 & 41.41 & 65.37 & 50.03\\
& BLIP4CIR \cite{BLIP4Cir} & BLIP & 43.49 & 67.31 & 42.09 & 67.33 & 41.76 & 64.28 & 46.61 & 70.32 & 55.40\\
\midrule
\multirow{19}{*}{Z-S}

& Image-Only & CLIP-L  & 7.97 & 17.43 & 5.25 & 13.63 & 10.54 & 20.65 & 8.10 & 18.01  \\ 
& Text-Only & CLIP-L  & 19.01 & 35.26 & 15.22 & 33.01 & 19.82 & 33.31 & 21.87 & 39.46 \\
& Image+Text & CLIP-L & 18.12 & 33.17 & 14.27 & 31.33 & 19.13 & 32.28 & 20.95 & 35.90 \\
& Pic2Word \cite{Saito_2023_CVPR} & CLIP-L & 24.7 & 43.7 & 20.0 & 40.2 & 26.2 & 43.6 & 27.9 & 47.4 & 34.2 \\
& SEARLE-XL* \cite{SEARLE} & CLIP-L & 25.56 & 46.23 & 20.48 & 43.13 & 26.89 & 45.58 & 29.32 & 49.97 \\
%& SEARLE-XL-OTI \cite{SEARLE} & CLIP-L & 27.61 & 47.90 & 21.57 & 44.47 & 30.37 & 47.49 & 30.90 & 51.76 & 37.75 \\
% & CompoDiff$\text{*}$ & \underline{37.36} & \underline{50.85} & \textbf{33.91} &\underline{47.85} & \underline{38.1} & 52.48 & \underline{40.07} & \underline{52.22} & \underline{44.10} \\
& TransAgg\textsuperscript{\textdagger} \cite{transagg} & CLIP-L & \textbf{28.57} & \underline{48.29} & \textbf{23.85} & 44.57 & \textbf{29.54} & \textbf{47.79} & \textbf{32.33} & \textbf{52.52}  \\
% & Context-I2W \cite{tang2023context} & CLIP-L & 27.8 & \textbf{48.9} & 23.1 & \textbf{45.3} & \textbf{29.7} & \textbf{48.6} & 30.6 & \textbf{52.9} \\
& SCOT (Ours) & CLIP-L & \underline{28.27} & 47.44 & \underline{23.69} & \underline{45.06} & \underline{29.09} & \underline{47.01} & \underline{32.02} & \underline{50.33}  \\

\cmidrule(lr){2-11}

& Image-Only & CLIP-B & 5.88 & 13.19 &  6.96 & 14.08 & 4.46 & 11.89 & 6.22 & 13.61 \\ 
& Text-Only & CLIP-B & 18.41 & 36.28 & 14.92 & 33.81 & 19.77 & 34.69 & 20.55 & 40.33 \\
& Image+Text & CLIP-B & 13.36 & 27.51 &  12.44 & 28.55 & 12.61 & 24.82 & 15.04 & 29.16  \\
& PALAVRA \cite{PALAVRA} & CLIP-B & 19.76 & 37.25 & 17.25 & 35.94 & 21.49 & 37.05 & 20.55 & 38.76 & 28.50 \\
& SEARLE* \cite{SEARLE} & CLIP-B & 22.89 & 42.53 & 18.54 & 39.51 & 24.44 & 41.61 & 18.54 & 39.51 \\
& TransAgg\textsuperscript{\textdagger} \cite{transagg} & CLIP-B & \underline{23.91} & \textbf{44.68} & \underline{19.44} & \textbf{42.04} & \underline{25.37} & \underline{42.69} & \underline{26.93} & \textbf{49.31} \\
& SCOT (Ours) & CLIP-B & \textbf{24.14} & \underline{43.44} & \textbf{19.73} & \underline{41.24} & \textbf{25.51} & \textbf{42.93} & \textbf{27.18} & \underline{46.14} \\

\cmidrule(lr){2-11}

& Image-Only & BLIP & 6.65 & 15.40 & 5.05 & 12.19 & 7.55 & 17.76 & 7.34 & 16.26 \\
& Text-Only & BLIP & 24.01 & 42.73 & 20.03 & 39.96 & 24.63 & 41.02 & 27.38 & 47.22  \\
& Image+Text & BLIP & 8.06 & 18.16 & 6.14 & 19.78 & 9.37 & 19.87 & 8.66 & 19.78  \\
& TransAgg\textsuperscript{\textdagger}\cite{transagg} & BLIP & \underline{26.95} & \underline{46.10} & \underline{21.67} & \underline{41.89} & \underline{28.07} & \underline{45.63} & \underline{31.11} & \underline{50.79}  \\
& SCOT (Ours) & BLIP & \textbf{30.68} & \textbf{51.33} & \textbf{26.42} & \textbf{49.23} & \textbf{30.91} &\textbf{49.65} & \textbf{34.72} & \textbf{55.12}  \\

\cmidrule(lr){2-11}

& Image-Only & BLIP-2 & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 \\
& Text Only & BLIP-2 & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31  \\
& Image+Text & BLIP-2 & \underline{29.21} & \underline{50.05} & \underline{23.30} & \underline{45.61} & \underline{32.82} & \underline{53.09} & \underline{31.51} & \underline{51.45}  \\
& SCOT (Ours) & BLIP-2 & \textbf{38.45} & \textbf{60.03} & \textbf{32.78} & \textbf{55.91} & \textbf{41.42} & \textbf{61.09} & \textbf{41.15} & \textbf{63.10} & \textbf{49.24} \\
\bottomrule
\end{tabular}
\vspace{0.3em}
\caption{\textbf{Results on FashionIQ.} 
The bottom portion of the table presents zero-shot results from our proposed approach compared against existing zero-shot methods, while the top portion presents results from existing fully-supervised approaches. *SEARLE results from inversion model. \textsuperscript{\textdagger}TransAgg results using frozen backbones. See supplementary material for more results.
}
\label{table:fashioniq}
\vspace{-1em}
\end{table*}

% & Image Only$^\dagger$ & 7.53 & 17.93 & 4.21 & 11.89 & 10.59 & 23.51 & 7.81 & 18.41 & 12.73 \\
% & Text Only$^\dagger$ & 24.68 & 43.59 & 20.77 & 41.64 & 25.95 & 42.83 & 27.33 & 46.31 & 34.13 \\
% & Image + Text$^\dagger$ & 29.21 & 50.05 & 23.3 & 45.61 & 32.82 & \underline{53.09} & 31.51 & 51.45 & 39.63 \\
